QRMeM: Unleash the Length Limitation through Question then Reflection Memory Mechanism

While large language models (LLMs) have made notable advancements in natural language processing, they continue to struggle with processing extensive text. Memory mechanism offers a flexible solution for managing long contexts, utilizing techniques such as compression, summarization, and structuring to facilitate nuanced and efficient handling of large volumes of text. However, existing techniques face challenges with static knowledge integration, leading to insufficient adaptation to task-specific needs and missing multi-segmentation relationships, which hinders the dynamic reorganization and logical combination of relevant segments during the response process. To address these issues, we introduce a novel strategy, Question then Reflection Memory Mechanism (QRMeM), incorporating a dual-structured memory pool. This pool synergizes static textual content with structured graph guidance, fostering a reflective trial-and-error approach for navigating and identifying relevant segments. Our evaluation across multiple-choice questions (MCQ) and multi-document question answering (Multi-doc QA) benchmarks showcases QRMeM enhanced performance compared to existing approaches.

==> prompt/question.tex <==
\begin{prompt}[title={The prompt used for Question Generation}, label=prompt:question]
Main text: \\
\"\"\"\\
\blue{[Segment Content]}\\
\"\"\"\\. Based on the main text, we have extracted several entities and relations: \\
\blue{[Entity Set]}
\blue{[Relation Set]}\\
The goal of this project is to generate questions based on the existing knowledge graph in order to help us have a more comprehensive understanding of the original documents and expand the content of this graph. When generating questions, please follow these steps: \\
1. Understand the content of the knowledge graph: Before formulating questions, it is important to have a deep understanding of the structure and information contained in the knowledge graph. Pay attention to entities (such as people, places, and events) in the graph and their relationships. \\
2. Diversity and complexity: Try to generate different types of questions, including but not limited to factual (\"Who is...?\"), descriptive (\"What is...?\"), comparative (\"How does ... differ from ...?\"), etc. 
3. Ensure accuracy: Questions should be based on accurate information from the document. Avoid introducing external knowledge or assumptions.\\
4. Consider gaps in the knowledge graph: Try to propose questions that can reveal current deficiencies or potential areas for expansion in the knowledge graph.\\
5. Clear and concise: Make sure that question statements are clear, concise, and easy to understand. Avoid overly complex or ambiguous expressions. 
\end{prompt}




